SketchGPT: Autoregressive Modeling for Sketch Generation and Recognition

We present SketchGPT, a flexible framework that employs a sequence-to-sequence autoregressive model for sketch generation, and completion, and an interpretation case study for sketch recognition. By mapping complex sketches into simplified sequences of abstract primitives, our approach significantly streamlines the input for autoregressive modeling. SketchGPT leverages the next token prediction objective strategy to understand sketch patterns, facilitating the creation and completion of drawings and also categorizing them accurately. This proposed sketch representation strategy aids in overcoming existing challenges of autoregressive modeling for continuous stroke data, enabling smoother model training and competitive performance. Our findings exhibit SketchGPT's capability to generate a diverse variety of drawings by adding both qualitative and quantitative comparisons with existing state-of-the-art, along with a comprehensive human evaluation study. The code and pretrained models will be released on our official GitHub.

==> tex/limitations.tex <==
Despite the strengths demonstrated by our model in sketch generation and completion tasks, as well as competitive performance in sketch classification, several limitations are worth noting, primarily stemming from our data representation methodology. 
Although the simplification of data through sketch approximation with primitives aids learning, it also results in information loss that adversely affects performance. Moreover, the absence of techniques like the Ramer-Douglas-Peucker (RDP) algorithm (\cite{Ha2018}, \cite{lin2020sketch}) to shorten the sequence length of the sketches difficults the model convergence, leading to worse performance. Since our approximation method already results in some loss of information, we opted against using additional algorithms like RDP, which could further simplify sketches and worsen the issue. 
Our methodology yields decent results when applied to datasets like QuickDraw, characterized by relatively simple sketches. But for more complex datasets such as TU-Berlin \cite{eitz2012humans}, the limitations of our data approximation through primitives become apparent; the substantial information loss significantly impacts the model's performance, particularly in tasks like sketch completion and generation. 
Moving forward, addressing these limitations demands the development of a better data representation strategy. Such a representation should aim to mitigate information loss while simultaneously reducing the maximum sequence length, which can impede model convergence and efficacy.

